Meta-Structures: The Search of Coherence in Collective Behaviours (without Physics)

This contribution shortly outlines and reviews a theoretical and computational approach for a theory of change concerning systems where it is not possible to apply the laws of motion ab initio. The concept of meta-structure relates to the emergence of forms of spatiotemporal coherences in collective behaviours intended as coherent sequences of multiple structures. The essential difference compared with traditional methods is the role of the cognitive design by the observer when identifying multiple mesoscopic variables. The goal is both to study the "change without physics" of the dynamics of change and to design non-catastrophic interventions having the purpose to induce, change, keep or restore collective behaviours by influencing -at the mesoscopic level -and not prescribing explicit rules and changes.

==> eptcsdata.tex <==
\providecommand{\firstpage}{35}
\providecommand{\publicationstatus}{A. Graudenzi, G. Caravagna, G. Mauri, M. Antoniotti (Eds.): \\Wivace 2013 - Italian Workshop on \\Artificial Life and Evolutionary Computation\\
EPTCS 130, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.130.6}{10.4204/EPTCS.130.6}}
\pdfoutput=1

